FACTIFY3M: A Benchmark for Multimodal Fact Verification with Explainability through 5W Question-Answering

Combating disinformation is one of the burning societal crises -- about 67% of the American population believes that disinformation produces a lot of uncertainty, and 10% of them knowingly propagate disinformation. Evidence shows that disinformation can manipulate democratic processes and public opinion, causing disruption in the share market, panic and anxiety in society, and even death during crises. Therefore, disinformation should be identified promptly and, if possible, mitigated. With approximately 3.2 billion images and 720,000 hours of video shared online daily on social media platforms, scalable detection of multimodal disinformation requires efficient fact verification. Despite progress in automatic text-based fact verification (e.g., FEVER, LIAR), the research community lacks substantial effort in multimodal fact verification. To address this gap, we introduce FACTIFY 3M, a dataset of 3 million samples that pushes the boundaries of the domain of fact verification via a multimodal fake news dataset, in addition to offering explainability through the concept of 5W question-answering. Salient features of the dataset include: (i) textual claims, (ii) ChatGPT-generated paraphrased claims, (iii) associated images, (iv) stable diffusion-generated additional images (i.e., visual paraphrases), (v) pixel-level image heatmap to foster image-text explainability of the claim, (vi) 5W QA pairs, and (vii) adversarial fake news stories.

==> 8_Discussion.tex <==
\section{Discussion}

Our work is centered around three major contributions: 

\begin{itemize}
    \item \textbf{Dataset of 1M multimodal fake news samples:} To foster fake news detection research, we have curated a dataset of 3M fake news articles and made it publicly available. These articles have been generated using the SoTA in text \cite{opt} and image generation \cite{rombach2021highresolution} models, followed by DAAM and CLIP-based reranking. The transcendental performance of these models has led to articles that are compelling and in most cases, virtually indistinguishable as real or fake to even experts.
    \item \textbf{5W explanation using QA pair generation:} We propose a new approach to modeling the process of fact verification as a process of 5W QA pair generation. This provides a structured and robust framework to help tease out the nuanced 5W components of the claim and thus, easily verify each of them.
    \item \textbf{Adversarial attack analysis:} We analyze the impact of an adversarial attack on the fact verification process. To motivate future research in fact verification systems, we make our dataset of adversarial examples available for researchers to benchmark their proposals. The dataset would offer a realistic evaluation of the researcher's proposal since the dissemination of fake news is already a rampant problem and is poised to only increase in scale with the proliferation of highly performant generative AI techniques. Furthermore, the significant challenges in programmatically detecting AI-generated artifacts add another layer of challenges.
    
\end{itemize}

Owing to the success of the diffusion model, using stable diffusion v2, we can successfully generate images that might confuse readers or reviewers into believing that the synthetically generated images might in fact be real-life photos.

Using DAAM, we are able to provide an image-level explanation. The cross-attention model allows us to break down each aspect of the image, thus allowing a human reader to interpret the validity of the image.

Applying 5W SRL to generate QA Pairs to verify authenticity provides textual explainability to verify the validity of the statements. \\ 

We are the first in the community to provide a multimodal fact verification dataset that is entailed with the explanation at the image and textual levels. 


